Federated Privacy-preserving Collaborative Filtering for On-Device Next App Prediction

In this study, we propose a novel SeqMF model to solve the problem of predicting the next app launch during mobile device usage. Although this problem can be represented as a classical collaborative filtering problem, it requires proper modification since the data are sequential, the user feedback is distributed among devices and the transmission of users' data to aggregate common patterns must be protected against leakage. According to such requirements, we modify the structure of the classical matrix factorization model and update the training procedure to sequential learning. Since the data about user experience are distributed among devices, the federated learning setup is used to train the proposed sequential matrix factorization model. One more ingredient of the proposed approach is a new privacy mechanism that guarantees the protection of the sent data from the users to the remote server. To demonstrate the efficiency of the proposed model we use publicly available mobile user behavior data. We compare our model with sequential rules and models based on the frequency of app launches. The comparison is conducted in static and dynamic environments. The static environment evaluates how our model processes sequential data compared to competitors. Therefore, the standard train-validation-test evaluation procedure is used. The dynamic environment emulates the real-world scenario, where users generate new data by running apps on devices, and evaluates our model in this case. Our experiments show that the proposed model provides comparable quality with other methods in the static environment. However, more importantly, our method achieves a better privacy-utility trade-off than competitors in the dynamic environment, which provides more accurate simulations of real-world usage.

==> text/seqmf.tex <==
\section{Sequence-aware Matrix Factorization for the next app prediction}
\label{sec:seqmf_next_app}
In this section, we design a new point-wise objective that incorporates knowledge about users' sequential behavior into the framework of the objective \eqref{eq:wrmf_vec}.
The main idea is to utilize the Markov Chain of length 1 \cite{Rendle_2010_FPMF}. However, typically it leads to a non-linear optimization task that can no longer be solved via ALS. The resulting objective is often a variant of the pair-wise BPR loss \cite{Rendle2012BPR} optimized with a GD-based method. 
Conversely, we do not have such freedom in our case as \emph{the ALS step is the necessary part of the optimization}, which forbids the use of non-linear loss functions. 

\subsection{Learning from Sequential Data}\label{sec:seqmf}
We start by defining a sequential user history as $\mathcal{H}_u^\ind{t} = \left(i_1^u, \dots, i_{|\mathcal{H}_u^\ind{t}|}^u\right)$, where $i_k^u \in \mathcal{I}_u$ a set of all available items of user $u$. 
In our case, $\mathcal{I}_u$ corresponds to the pool of only installed apps on the user device, which is much smaller than the number of all unique apps in the app store.

Let us rewrite \eqref{eq:wrmf_vec} in a more general form:
\begin{equation}\label{eq:gen_loss}
    \mathcal{L}(\matr{\Theta}, t) = \frac{1}{2}\sum_u \left\|\vect{r}_u(\matr{\Theta}, t)-\vect{a}_u^\ind{t}\right\|^2_{\matr{C}_u^\ind{t}} + \frac{\lambda}{2}\left\|\matr{\Theta}\right\|^2, \quad \matr{\Theta} = \left\{\{\vect{p}_u\}_{u=1}^M,\{\vect{q}_i\}_{i=1}^N\right\},
\end{equation}
where $r_u(\matr{\Theta}, t)$ is expected to capture both long-term and short-term effects. 
Parameter $t$ controls how many events from history are considered for calculations, e.g. all up to moment $t$.

The relevance prediction rule \eqref{eq:prediction_rule_base} is now extended with an additional term responsible for short-term effects:
\begin{equation}
    \label{eq:prediction-rule}
    \vect{r}_u(\matr{\Theta}, t) =
    \matr{Q}\vect{p}_u + \vect{h}_u^\ind{t}(\matr{Q}) = 
    \matr{Q}\vect{p}_u + \diag{\matr{S}_u^\ind{t}\matr {Q}\matr{Q}^\top}
\end{equation}
where the ``design matrix'' $\matr{S}_u^\ind{t}$ encodes relative frequency weights corresponding to transition to item $i$ from some previous item $j$ in user history. 
It can be defined as:
\begin{equation}
    \label{eq:design_matrix}
    \left(\matr{S}_u^\ind{t}\right)_{ij}=
    \ddfrac{\sum_{k=2}^{|\mathcal{H}_u^\ind{t}|}\mathds{1}[j\rightarrow i]\mathds{1}[i_{k-1}^u=j] \mathds{1}[i_k^u=i]}{\sum_{k=2}^{|\mathcal{H}_u^\ind{t}|}\mathds{1}[i_{k-1}^u=i]}
\end{equation}
where $\mathds{1}[j\rightarrow i]$ equals $1$ if there was a transition to item $i$ from item $j$ otherwise 0, $\mathds{1}[m=n]$ equals $1$ if $m=n$ otherwise 0.

For example, let a user $u$ has the following history of interactions: $\mathcal{H}_u^\ind{t} = \left(a, b, c, a, a, b, a, c\right)$. The resulting matrix $\matr{S}_u^\ind{t}$ would look like:
\begin{equation}
\matr{S}_u^\ind{t} = \begin{blockarray}{cccc}
        a & b & c & \\
       \begin{block}{(ccc)c}
         \frac{1}{4} & \frac{2}{4}  & \frac{1}{4} & a \\
         \frac{1}{2} & 0 & \frac{1}{2} & b \\
         \frac{1}{1} & 0 & 0 & c\\
       \end{block}
     \end{blockarray}
\end{equation}
because e.g. for $\left(\matr{S}_u^\ind{t}\right)_{ab}$ we can count 2 sequential co-occurrences of $(a, b)$ and 4 occurrences of $a$.

Elements of the short-term preference part $\vect{h}_u^\ind{t}(\matr{Q})$ define the affinity of items from the past to the current target item (the target is simply a candidate for the next item prediction). 
Following the ideas from previous research on sequence-aware MF \cite{McAuley_2016_Fossil}, we will measure the affinity between target item $i$ and some preceding item $j$ via scalar product $\vect{q}_i^\top \vect{q}_j$. 
In order to account for the preceding item for the target item $i$, we define the corresponding elements of $\vect{h}_u^\ind{t}(\matr{Q})$ as:
\begin{equation}\label{eq:samf_group}
    \left(\vect{h}_u^\ind{t}\right)_i=
    \sum_{j=1}^N\left(\matr{S}_u^\ind{t}\right)_{ij}\vect{q}_i^\top\vect{q}_j
\end{equation}
In order to better account for changes in the global dynamics of app usage frequencies, one has to restrict a history period. 
It can be done using a time window of the most recent events e.g. several weeks or months depending on available data. 
Smaller $t$ improves computational performance while larger $t$ may help discover longer range correlations between events that do not immediately follow one another. In our experiments, we use all the data up to $t$ as the datasets are small.

\subsection{Model Updates}
The updates for local user factors $\vect{p}_u$ using ALS scheme can be computed from \eqref{eq:gen_loss} as follows:
\begin{equation}\label{eq:p_u}
\vect{p}_{u} = \left(\matr{Q}^\top \matr{C}_{u}^\ind{t}\matr{Q} + \lambda \matr{I} \right)^{-1}\matr{Q}^\top  
\matr{C}_{u}^\ind{t}
\left(\vect{a}_{u}^\ind{t} -  \diag{\matr{S}_u^\ind{t}\matr{Q}\matr{Q}^\top}\right).
\end{equation}
Recall that factors $\vect{p}_u$ are responsible for the long-term preferences (\sref{sec::federated_framework}). 
From the right-hand side of~\eqref{eq:p_u}, one can see that the influence of the long-term preferences encoded in $\vect{a}_u$ is compensated with the short-term sequential dynamics represented by $\diag{\matr{S}_u^\ind{t}\matr{Q}\matr{Q}^\top}$. 
This is exactly the behavior we planned to achieve.

Likewise, the updates for the global preferences matrix $\matr{Q}$ are calculated based on the gradient of the objective function with respect to the matrix $\matr{Q}$: 
\begin{equation}
    \label{eq:seqmf_Q_update}
    \ddfrac{\partial \mathcal{L}}{\partial \matr{Q}} = \sum_{u = 1}^{M}
    \matr{D}_u^\ind{t} \vect{e}_N\vect{p}_u^\top + \left(\matr{D}_u^\ind{t}\matr{S}_u^\ind{t} + {\matr{S}_u^\ind{t}}^\top\matr{D}_u^\ind{t}\right)\matr{Q} + \lambda \matr{Q},
\end{equation}
where $\matr{D}_u^\ind{t} = \diag{\matr{C}_{u}^\ind{t}\left(\vect{r}_{u}(\matr{\Theta}, t) - \vect{a}_{u}^\ind{t}\right)}$, $\vect{e}_N$~--- vector of ones of size $N$.
This gradient can be used in gradient-based optimizers to update the global preference matrix $\matr{Q}$. 
We call the resulting model \textbf{SeqMF}.

\subsection{SeqMF Inference}
The prediction rule \eqref{eq:prediction-rule} is designed to facilitate proper learning of app co-occurrence statistics from a history of user actions. 
While necessary for the training, it has to be modified for the prediction step to make inference more lightweight.

Hence, we adopt a few simpler rules for the prediction that only take into account the current user session and reweight the contribution of items from it. 
One of them is based on a simple aggregation:
\begin{equation}
    \label{eq:sum_prediction}
\operatorname{score}_{\mathrm{sum}}(u, i, s) = \vect{q}_{i}^\top\left(\vect{p}_{u} + \sum_{j=1}^{|s|}\vect{q}_{j}\right),
\end{equation}
where $|s|$ is the length of item session $s$. 
Another one is based on averaging: 
\begin{equation}
    \label{eq:av_prediction}
\operatorname{score}_{\mathrm{av}}(u, i, s)=\vect{q}_{i}^\top\left(\vect{p}_{u} + \dfrac{1}{|s|} \sum_{j=1}^{|s|}\vect{q}_{j}\right)
\end{equation}

In order to find top-n candidates with use equation \eqref{eq:prediction} with aforementioned score functions. In the experiments we used $\operatorname{score}_{\mathrm{sum}}(u, i, s)$ as it showed better quality.

 

\subsection{Confidence-based Weighting Coefficients}\label{sec:confidence}
The essence of confidence-based weighting approaches is to assign proper importance weights to discrepancies between prediction and ground truth on both observed and unobserved interactions while training a model. 
That way the model is expected to learn better representations and capture underlying behavioral patterns more accurately. 
Popular weighting schemes (e.g., \cite{Koren_2008_ICF}) assign small uniform weights on unobserved data (emphasizing the lower contribution of such examples in the learning process) and higher data-dependent weights on observed entries. 
Such schemes proved to be effective in practice for standard CF tasks \cite{Koren_2008_ICF, Li_CF_Wights_2018}. 
However, preliminary experiments showed that standard weighting schemes did not work for our settings where \emph{the main goal is to predict the next app from the pool of available apps on user device}.

%Let us define the notion of \emph{active} and \emph{inactive} apps. Active apps were installed on user device and used at least once throughout the available user history (or within a certain time interval of sufficient length). Inactive apps are all other apps that were either never installed or never used on a device (at least within a given history $\mathcal{H}^\ind{t}_u$).

%Therefore, there are two possibilities for unobserved interactions. Not seeing an active app in the current session means that the user has specifically chosen to use some other app here. It hints that the context (e.g., previously launched apps) is not appropriate for this app. We argue that this is a strong signal, and the contribution of this unobserved interaction must still be relatively high, especially if the app is frequently used by the user in general. Ideally, such examples should drive better learning of the sequential parameters of the model (that are responsible for the context). Conversely, the long-term factors should not be influenced much by these examples.On the other hand, for an unobserved inactive app, there is no possibility to observe it until it is installed by a user. As we may never know the reason for this app being unused, this type of feedback is trivial and should have a much lower contribution to the learning process.

%Hence, we have two types of negative feedback that must be associated with different types of confidence weights. 
%We also note that the negative feedback for active apps by its nature is similar to positive feedback. 
%Thus, we can use the same confidence weighting scheme for both types of feedback in the case of active apps. 
Following ideas on frequency-based weighting \cite{He_FMF_2017}, we propose the following expression for confidence:
\begin{equation}\label{eq:rel_freq}
    c_{u,i} = \frac{f^\gamma_{u,i} + \alpha}{\sum_j f^\gamma_{u,j} + \alpha N},
\end{equation}
where $f_{u,i}$ is a launch frequency of item $i$ in the history of user $u$, and $\alpha, \gamma$ are found during hyper-parameters search. 
By modifying relative frequencies $f_{u,i}$ with $\alpha$-additive (Laplace) smoothing~\cite{Valcarce_2016_Smoothing}
we make the confidence values on inactive apps a small non-zero constant, which is fully compatible with conventional weighted ALS-based approaches.
Note that setting $\alpha$ not to zero leads to increase in computational cost due to implementation peculiarities.
